A Systematic Study of Performance Disparities in Multilingual Task-Oriented Dialogue Systems

Achieving robust language technologies that can perform well across the world's many languages is a central goal of multilingual NLP. In this work, we take stock of and empirically analyse task performance disparities that exist between multilingual task-oriented dialogue (ToD) systems. We first define new quantitative measures of absolute and relative equivalence in system performance, capturing disparities across languages and within individual languages. Through a series of controlled experiments, we demonstrate that performance disparities depend on a number of factors: the nature of the ToD task at hand, the underlying pretrained language model, the target language, and the amount of ToD annotated data. We empirically prove the existence of the adaptation and intrinsic biases in current ToD systems: e.g., ToD systems trained for Arabic or Turkish using annotated ToD data fully parallel to English ToD data still exhibit diminished ToD task performance. Beyond providing a series of insights into the performance disparities of ToD systems in different languages, our analyses offer practical tips on how to approach ToD data collection and system development for new languages.

==> 07_proposal.tex <==
Developing a task-oriented dialogue system from scratch requires the acquisition of a large-scale in-domain dataset, a laborious and expensive endeavour that relies on domain expertise and substantial time investment~\cite{Shah:2018naacl, Larson:2022arxiv, multi3woz}. As a result, progress in developing task-oriented systems until recently has been limited only to a small number of high-resource languages such as English and Chinese~\cite{Razumovskaia:2022survey}.

On the other hand, recent advances in pre-trained multilingual language models, such as mBERT~\cite{devlin2018bert}, XLM-R~\cite{conneau-etal-2020-unsupervised}, or mT5~\cite{xue2020mt5}, have conceptually enabled cross-lingual transfer between any two languages seen in pretraining~\cite{hu2020xtreme} or even to unseen languages~\cite{ansell2021mad}. Consequently, these models offer the opportunity to develop systems in target languages without the need for exhaustive, language-specific dataset collection.
\songbo{I didn't pay attention to the citations here. Many of them are missing.}

With the challenges posed and the availability of state-of-the-art multilingual models, this paper aims to address the following research questions:
\begin{enumerate*}
    \item Is language-specific data still necessary for developing a dialogue system in a new language?
    \item What is the required quantity of data to construct a high-performing dialogue system in a new language?
    \item Which strategy offers optimal cost-efficiency for creating task-oriented dialogue data in a new language?
\end{enumerate*}
By investigating these research questions, we aim to shed light on the viability of leveraging multilingual models and explore efficient data collection approaches for developing dialogue systems for the next 100 languages equitably.\songbo{I think we can put a big name here. I have heard many times that the goal is to develop language technologies for the next 100 languages. And also we could use this to argue that we want to train a system that performs similarly to a system trained with a full in-domain dataset, motivating our experimental setup.}
\han{haha I like 100 langs}

Our experimental study aims to investigate the development of \textit{equitable} dialogue systems in both resource-rich languages, like English (\eng), and resource-scarce languages, such as Arabic (\ara). To accomplish this, we leverage a multilingual dialogue model denoted as $M$ and an English dialogue dataset represented as $\mathbbm{D}^{\eng}$. By training $M$ on $\mathbbm{D}^{\eng}$, we are able to specialise the model into a language-specific variant referred to as $M^{\eng}$. Subsequently, we evaluate the fine-tuned dialogue model by measuring its performance using a task-specific evaluation score denoted as $s^{\eng} = \operatorname{S}(M^{\eng}, \mathbbm{D}^{\eng})$.

To ensure the development of an equitable dialogue system, we assume the existence of a training dataset in the target language, denoted as $\mathbbm{D}^{\ara}$, which is fully multi-parallel to $\mathbbm{D}^{\eng}$. Subsequently, a language-specific model $M^{\ara}$ is trained on $\mathbbm{D}^{\eng}$, which achieves a task-specific score of $s^{\ara} = \operatorname{S}(M^{\ara}, \mathbbm{D}^{\ara})$. It worth noting that this paper focus on data creation and assume the multilingual models $M$ performs fairly for each language.

However, as mentioned earlier, creating a fully multi-parallel dataset for all target languages is impractical. In this study, we explore a more realistic scenario where only a limited subset of the target language dataset is available. Specifically, we assume the existence of $\mathbbm{D}_{subset}^{\ara} \subset \mathbbm{D}^{\ara}$. We define the model $M_{subset}^{\ara}$ trained on $\mathbbm{D}_{subset}^{\ara}$ as achieving \textit{equitable} performance if $s_{subset}^{\ara} \geq (1-\theta)*s^{\ara}$, where $s_{subset}^{\ara} = \operatorname{S}(M_{subset}^{\ara}, \mathbbm{D}_{subset}^{\ara})$ and $\theta \in [0,1]$. This paper focuses on investigating the optimal strategies for data creation, aiming to achieve equitable performance in the target language while minimising the cost associated with data creation.\songbo{I didn't check the notation carefully, but I hope the main idea is not confusing.}

Experiment 1: We show the performance gap between fully supervised training and zero-shot cross-lingual transfer performance. Already done. :) Answering research question 1.

Experiment 2: We show how much data we need to achieve equitable performance. Based on the figure we have seen during the meeting, it is roughly about 20\%.

Experiment 3: Could we do better? We have to experiment with different subsets of our target language dataset and find the optimal subset with the lowerest cost (number of dialogues?) that achieves near fully supervised performance.

Important side experiments: run a subset of the most important experiments 1) with a larger model (mT5-large) to check that the gap remains even with larger models; 2) with an arguably fairer pretraining model (umT5; \url{https://twitter.com/hwchung27/status/1648790668628852738}) to see how it reflects of ToD performance.








